Expandable Factor Analysis

Bayesian sparse factor models have proven useful for characterizing dependence in multivariate data, but scaling computation to large numbers of samples and dimensions is problematic. We propose expandable factor analysis for scalable inference in factor models when the number of factors is unknown. The method relies on a continuous shrinkage prior for efficient maximum a posteriori estimation of a low-rank and sparse loadings matrix. The structure of the prior leads to an estimation algorithm that accommodates uncertainty in the number of factors. We propose an information criterion to select the hyperparameters of the prior. Expandable factor analysis has better false discovery rates and true positive rates than its competitors across diverse simulations. We apply the proposed approach to a gene expression study of aging in mice, illustrating superior results relative to four competing methods.

==> Definitions.tex <==
\RequirePackage{latexsym}
\RequirePackage{amsmath}
%\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}             %
\RequirePackage{soul}

%%% MW %%%%

\newcommand{\mnote}[1]{{\bf\large *}\marginpar{\tiny#1}}
\newcommand{\dnote}[1]{{\bf\large +}\marginpar{\tiny#1}}
%\newcommand{\note}[1]{{\bf #1}}


%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

% \DeclareMathOperator{\ab}{\mathbf{a}}
% \DeclareMathOperator{\bb}{\mathbf{b}}
% \DeclareMathOperator{\cb}{\mathbf{c}}
% \DeclareMathOperator{\db}{\mathbf{d}}
% \DeclareMathOperator{\eb}{\mathbf{e}}
% \DeclareMathOperator{\fb}{\mathbf{f}}
% \DeclareMathOperator{\gb}{\mathbf{g}}
% \DeclareMathOperator{\hb}{\mathbf{h}}
% \DeclareMathOperator{\ib}{\mathbf{i}}
% \DeclareMathOperator{\jb}{\mathbf{j}}
% \DeclareMathOperator{\kb}{\mathbf{k}}
% \DeclareMathOperator{\lb}{\mathbf{l}}
% \DeclareMathOperator{\mb}{\mathbf{m}}
% \DeclareMathOperator{\nbb}{\mathbf{n}}
% \DeclareMathOperator{\ob}{\mathbf{o}}
% \DeclareMathOperator{\pb}{\mathbf{p}}
% \DeclareMathOperator{\qb}{\mathbf{q}}
% \DeclareMathOperator{\rb}{\mathbf{r}}
% \DeclareMathOperator{\sbb}{\mathbf{s}}
% \DeclareMathOperator{\tb}{\mathbf{t}}
% \DeclareMathOperator{\ub}{\mathbf{u}}
% \DeclareMathOperator{\vb}{\mathbf{v}}
% \DeclareMathOperator{\wb}{\mathbf{w}}
% \DeclareMathOperator{\xb}{\mathbf{x}}
% \DeclareMathOperator{\yb}{\mathbf{y}}
% \DeclareMathOperator{\zb}{\mathbf{z}}

\DeclareMathOperator{\ab}{\mathbold{a}}
\DeclareMathOperator{\bb}{\mathbold{b}}
\DeclareMathOperator{\cb}{\mathbold{c}}
\DeclareMathOperator{\db}{\mathbold{d}}
\DeclareMathOperator{\eb}{\mathbold{e}}
\DeclareMathOperator{\fb}{\mathbold{f}}
\DeclareMathOperator{\gb}{\mathbold{g}}
\DeclareMathOperator{\hb}{\mathbold{h}}
\DeclareMathOperator{\ib}{\mathbold{i}}
\DeclareMathOperator{\jb}{\mathbold{j}}
\DeclareMathOperator{\kb}{\mathbold{k}}
\DeclareMathOperator{\lb}{\mathbold{l}}
\DeclareMathOperator{\mb}{\mathbold{m}}
\DeclareMathOperator{\nbb}{\mathbold{n}}
\DeclareMathOperator{\ob}{\mathbold{o}}
\DeclareMathOperator{\pb}{\mathbold{p}}
\DeclareMathOperator{\qb}{\mathbold{q}}
\DeclareMathOperator{\rb}{\mathbold{r}}
\DeclareMathOperator{\sbb}{\mathbold{s}}
\DeclareMathOperator{\tb}{\mathbold{t}}
\DeclareMathOperator{\ub}{\mathbold{u}}
\DeclareMathOperator{\vb}{\mathbold{v}}
\DeclareMathOperator{\wb}{\mathbold{w}}
\DeclareMathOperator{\xb}{\mathbold{x}}
\DeclareMathOperator{\yb}{\mathbold{y}}
\DeclareMathOperator{\zb}{\mathbold{z}}

% \DeclareMathOperator{\atilde}{\tilde{a}}
% \DeclareMathOperator{\btilde}{\tilde{b}}
% \DeclareMathOperator{\ctilde}{\tilde{c}}
% \DeclareMathOperator{\dtilde}{\tilde{d}}
% \DeclareMathOperator{\etilde}{\tilde{e}}
% \DeclareMathOperator{\ftilde}{\tilde{f}}
% \DeclareMathOperator{\gtilde}{\tilde{g}}
% \DeclareMathOperator{\htilde}{\tilde{h}}
% \DeclareMathOperator{\itilde}{\tilde{i}}
% \DeclareMathOperator{\jtilde}{\tilde{j}}
% \DeclareMathOperator{\ktilde}{\tilde{k}}
% \DeclareMathOperator{\ltilde}{\tilde{l}}
% \DeclareMathOperator{\mtilde}{\tilde{m}}
% \DeclareMathOperator{\ntilde}{\tilde{n}}
% \DeclareMathOperator{\otilde}{\tilde{o}}
% %
% \DeclareMathOperator{\qtilde}{\tilde{q}}
% \DeclareMathOperator{\rtilde}{\tilde{r}}
% \DeclareMathOperator{\stilde}{\tilde{s}}
% \DeclareMathOperator{\ttilde}{\tilde{t}}
% \DeclareMathOperator{\utilde}{\tilde{u}}
% \DeclareMathOperator{\vtilde}{\tilde{v}}
% \DeclareMathOperator{\wtilde}{\tilde{w}}
% \DeclareMathOperator{\xtilde}{\tilde{x}}
% \DeclareMathOperator{\ytilde}{\tilde{y}}
% \DeclareMathOperator{\ztilde}{\tilde{z}}

\DeclareMathOperator{\abar}{\bar{\ab}}
\DeclareMathOperator{\bbar}{\bar{\bb}}
\DeclareMathOperator{\cbar}{\bar{\cb}}
\DeclareMathOperator{\dbar}{\bar{\db}}
\DeclareMathOperator{\ebar}{\bar{\eb}}
\DeclareMathOperator{\fbar}{\bar{\fb}}
\DeclareMathOperator{\gbar}{\bar{\gb}}
\DeclareMathOperator{\hbbar}{\bar{\hb}}
\DeclareMathOperator{\ibar}{\bar{\ib}}
\DeclareMathOperator{\jbar}{\bar{\jb}}
\DeclareMathOperator{\kbar}{\bar{\kb}}
\DeclareMathOperator{\lbar}{\bar{\lb}}
\DeclareMathOperator{\mbar}{\bar{\mb}}
\DeclareMathOperator{\nbar}{\bar{\nbb}}
\DeclareMathOperator{\obar}{\bar{\ob}}
\DeclareMathOperator{\pbar}{\bar{\pb}}
\DeclareMathOperator{\qbar}{\bar{\qb}}
\DeclareMathOperator{\rbar}{\bar{\rb}}
\DeclareMathOperator{\sbar}{\bar{\sbb}}
\DeclareMathOperator{\tbar}{\bar{\tb}}
\DeclareMathOperator{\ubar}{\bar{\ub}}
\DeclareMathOperator{\vbar}{\bar{\vb}}
\DeclareMathOperator{\wbar}{\bar{\wb}}
\DeclareMathOperator{\xbar}{\bar{\xb}}
\DeclareMathOperator{\ybar}{\bar{\yb}}
\DeclareMathOperator{\zbar}{\bar{\zb}}

\DeclareMathOperator{\ahat}{\widehat{a}}
\DeclareMathOperator{\bhat}{\widehat{b}}
\DeclareMathOperator{\chat}{\widehat{c}}
\DeclareMathOperator{\dhat}{\widehat{d}}
\DeclareMathOperator{\ehat}{\widehat{e}}
\DeclareMathOperator{\fhat}{\widehat{f}}
\DeclareMathOperator{\ghat}{\widehat{g}}
\DeclareMathOperator{\hbhat}{\widehat{h}}
\DeclareMathOperator{\ihat}{\widehat{i}}
\DeclareMathOperator{\jhat}{\widehat{j}}
\DeclareMathOperator{\khat}{\widehat{k}}
\DeclareMathOperator{\lhat}{\widehat{l}}
\DeclareMathOperator{\mhat}{\widehat{m}}
\DeclareMathOperator{\nhat}{\widehat{n}}
\DeclareMathOperator{\ohat}{\widehat{o}}
\DeclareMathOperator{\phat}{\widehat{p}}
\DeclareMathOperator{\qhat}{\widehat{q}}
\DeclareMathOperator{\rhat}{\widehat{r}}
\DeclareMathOperator{\shat}{\widehat{s}}
\DeclareMathOperator{\that}{\widehat{t}}
\DeclareMathOperator{\uhat}{\widehat{u}}
\DeclareMathOperator{\vhat}{\widehat{v}}
\DeclareMathOperator{\what}{\widehat{w}}
\DeclareMathOperator{\xhat}{\widehat{x}}
\DeclareMathOperator{\yhat}{\widehat{y}}
\DeclareMathOperator{\zhat}{\widehat{z}}

% \DeclareMathOperator{\Ab}{\mathbf{A}}
% \DeclareMathOperator{\Bb}{\mathbf{B}}
% \DeclareMathOperator{\Cb}{\mathbf{C}}
% \DeclareMathOperator{\Db}{\mathbf{D}}
% \DeclareMathOperator{\Eb}{\mathbf{E}}
% \DeclareMathOperator{\Gb}{\mathbf{G}}
% \DeclareMathOperator{\Hb}{\mathbf{H}}
% \DeclareMathOperator{\Ib}{\mathbf{I}}
% \DeclareMathOperator{\Jb}{\mathbf{J}}
% \DeclareMathOperator{\Kb}{\mathbf{K}}
% \DeclareMathOperator{\Lb}{\mathbf{L}}
% \DeclareMathOperator{\Mb}{\mathbf{M}}
% \DeclareMathOperator{\Nb}{\mathbf{N}}
% \DeclareMathOperator{\Ob}{\mathbf{O}}
% \DeclareMathOperator{\Pb}{\mathbf{P}}
% \DeclareMathOperator{\Qb}{\mathbf{Q}}
% \DeclareMathOperator{\Rb}{\mathbf{R}}
% \DeclareMathOperator{\Sbb}{\mathbf{S}}
% \DeclareMathOperator{\Tb}{\mathbf{T}}
% \DeclareMathOperator{\Ub}{\mathbf{U}}
% \DeclareMathOperator{\Vb}{\mathbf{V}}
% \DeclareMathOperator{\Wb}{\mathbf{W}}
% \DeclareMathOperator{\Xb}{\mathbf{X}}
% \DeclareMathOperator{\Yb}{\mathbf{Y}}
% \DeclareMathOperator{\Zb}{\mathbf{Z}} 

\DeclareMathOperator{\Ab}{\mathbold{A}}
\DeclareMathOperator{\Bb}{\mathbold{B}}
\DeclareMathOperator{\Cb}{\mathbold{C}}
\DeclareMathOperator{\Db}{\mathbold{D}}
\DeclareMathOperator{\Eb}{\mathbold{E}}
\DeclareMathOperator{\Gb}{\mathbold{G}}
\DeclareMathOperator{\Hb}{\mathbold{H}}
\DeclareMathOperator{\Ib}{\mathbold{I}}
\DeclareMathOperator{\Jb}{\mathbold{J}}
\DeclareMathOperator{\Kb}{\mathbold{K}}
\DeclareMathOperator{\Lb}{\mathbold{L}}
\DeclareMathOperator{\Mb}{\mathbold{M}}
\DeclareMathOperator{\Nb}{\mathbold{N}}
\DeclareMathOperator{\Ob}{\mathbold{O}}
\DeclareMathOperator{\Pb}{\mathbold{P}}
\DeclareMathOperator{\Qb}{\mathbold{Q}}
\DeclareMathOperator{\Rb}{\mathbold{R}}
\DeclareMathOperator{\Sbb}{\mathbold{S}}
\DeclareMathOperator{\Tb}{\mathbold{T}}
\DeclareMathOperator{\Ub}{\mathbold{U}}
\DeclareMathOperator{\Vb}{\mathbold{V}}
\DeclareMathOperator{\Wb}{\mathbold{W}}
\DeclareMathOperator{\Xb}{\mathbold{X}}
\DeclareMathOperator{\Yb}{\mathbold{Y}}
\DeclareMathOperator{\Zb}{\mathbold{Z}} 
\DeclareMathOperator{\Abar}{\bar{A}}
\DeclareMathOperator{\Bbar}{\bar{B}}
\DeclareMathOperator{\Cbar}{\bar{C}}
\DeclareMathOperator{\Dbar}{\bar{D}}
\DeclareMathOperator{\Ebar}{\bar{E}}
\DeclareMathOperator{\Fbar}{\bar{F}}
\DeclareMathOperator{\Gbar}{\bar{G}}
\DeclareMathOperator{\Hbar}{\bar{H}}
\DeclareMathOperator{\Ibar}{\bar{I}}
\DeclareMathOperator{\Jbar}{\bar{J}}
\DeclareMathOperator{\Kbar}{\bar{K}}
\DeclareMathOperator{\Lbar}{\bar{L}}
\DeclareMathOperator{\Mbar}{\bar{M}}
\DeclareMathOperator{\Nbar}{\bar{N}}
\DeclareMathOperator{\Obar}{\bar{O}}
\DeclareMathOperator{\Pbar}{\bar{P}}
\DeclareMathOperator{\Qbar}{\bar{Q}}
\DeclareMathOperator{\Rbar}{\bar{R}}
\DeclareMathOperator{\Sbar}{\bar{S}}
\DeclareMathOperator{\Tbar}{\bar{T}}
\DeclareMathOperator{\Ubar}{\bar{U}}
\DeclareMathOperator{\Vbar}{\bar{V}}
\DeclareMathOperator{\Wbar}{\bar{W}}
\DeclareMathOperator{\Xbar}{\bar{X}}
\DeclareMathOperator{\Ybar}{\bar{Y}}
\DeclareMathOperator{\Zbar}{\bar{Z}}

\DeclareMathOperator{\Abbar}{\bar{\Ab}}
\DeclareMathOperator{\Bbbar}{\bar{\Bb}}
\DeclareMathOperator{\Cbbar}{\bar{\Cb}}
\DeclareMathOperator{\Dbbar}{\bar{\Db}}
\DeclareMathOperator{\Ebbar}{\bar{\Eb}}
\DeclareMathOperator{\Fbbar}{\bar{\Fb}}
\DeclareMathOperator{\Gbbar}{\bar{\Gb}}
\DeclareMathOperator{\Hbbar}{\bar{\Hb}}
\DeclareMathOperator{\Ibbar}{\bar{\Ib}}
\DeclareMathOperator{\Jbbar}{\bar{\Jb}}
\DeclareMathOperator{\Kbbar}{\bar{\Kb}}
\DeclareMathOperator{\Lbbar}{\bar{\Lb}}
\DeclareMathOperator{\Mbbar}{\bar{\Mb}}
\DeclareMathOperator{\Nbbar}{\bar{\Nb}}
\DeclareMathOperator{\Obbar}{\bar{\Ob}}
\DeclareMathOperator{\Pbbar}{\bar{\Pb}}
\DeclareMathOperator{\Qbbar}{\bar{\Qb}}
\DeclareMathOperator{\Rbbar}{\bar{\Rb}}
\DeclareMathOperator{\Sbbar}{\bar{\Sb}}
\DeclareMathOperator{\Tbbar}{\bar{\Tb}}
\DeclareMathOperator{\Ubbar}{\bar{\Ub}}
\DeclareMathOperator{\Vbbar}{\bar{\Vb}}
\DeclareMathOperator{\Wbbar}{\bar{\Wb}}
\DeclareMathOperator{\Xbbar}{\bar{\Xb}}
\DeclareMathOperator{\Ybbar}{\bar{\Yb}}
\DeclareMathOperator{\Zbbar}{\bar{\Zb}}

\DeclareMathOperator{\Ahat}{\widehat{A}}
\DeclareMathOperator{\Bhat}{\widehat{B}}
\DeclareMathOperator{\Chat}{\widehat{C}}
\DeclareMathOperator{\Dhat}{\widehat{D}}
\DeclareMathOperator{\Ehat}{\widehat{E}}
\DeclareMathOperator{\Fhat}{\widehat{F}}
\DeclareMathOperator{\Ghat}{\widehat{G}}
\DeclareMathOperator{\Hhat}{\widehat{H}}
\DeclareMathOperator{\Ihat}{\widehat{I}}
\DeclareMathOperator{\Jhat}{\widehat{J}}
\DeclareMathOperator{\Khat}{\widehat{K}}
\DeclareMathOperator{\Lhat}{\widehat{L}}
\DeclareMathOperator{\Mhat}{\widehat{M}}
\DeclareMathOperator{\Nhat}{\widehat{N}}
\DeclareMathOperator{\Ohat}{\widehat{O}}
\DeclareMathOperator{\Phat}{\widehat{P}}
\DeclareMathOperator{\Qhat}{\widehat{Q}}
\DeclareMathOperator{\Rhat}{\widehat{R}}
\DeclareMathOperator{\Shat}{\widehat{S}}
\DeclareMathOperator{\That}{\widehat{T}}
\DeclareMathOperator{\Uhat}{\widehat{U}}
\DeclareMathOperator{\Vhat}{\widehat{V}}
\DeclareMathOperator{\What}{\widehat{W}}
\DeclareMathOperator{\Xhat}{\widehat{X}}
\DeclareMathOperator{\Yhat}{\widehat{Y}}
\DeclareMathOperator{\Zhat}{\widehat{Z}}

\DeclareMathOperator{\Abhat}{\widehat{\Ab}}
\DeclareMathOperator{\Bbhat}{\widehat{\Bb}}
\DeclareMathOperator{\Cbhat}{\widehat{\Cb}}
\DeclareMathOperator{\Dbhat}{\widehat{\Db}}
\DeclareMathOperator{\Ebhat}{\widehat{\Eb}}
\DeclareMathOperator{\Fbhat}{\widehat{\Fb}}
\DeclareMathOperator{\Gbhat}{\widehat{\Gb}}
\DeclareMathOperator{\Hbhat}{\widehat{\Hb}}
\DeclareMathOperator{\Ibhat}{\widehat{\Ib}}
\DeclareMathOperator{\Jbhat}{\widehat{\Jb}}
\DeclareMathOperator{\Kbhat}{\widehat{\Kb}}
\DeclareMathOperator{\Lbhat}{\widehat{\Lb}}
\DeclareMathOperator{\Mbhat}{\widehat{\Mb}}
\DeclareMathOperator{\Nbhat}{\widehat{\Nb}}
\DeclareMathOperator{\Obhat}{\widehat{\Ob}}
\DeclareMathOperator{\Pbhat}{\widehat{\Pb}}
\DeclareMathOperator{\Qbhat}{\widehat{\Qb}}
\DeclareMathOperator{\Rbhat}{\widehat{\Rb}}
\DeclareMathOperator{\Sbhat}{\widehat{\Sb}}
\DeclareMathOperator{\Tbhat}{\widehat{\Tb}}
\DeclareMathOperator{\Ubhat}{\widehat{\Ub}}
\DeclareMathOperator{\Vbhat}{\widehat{\Vb}}
\DeclareMathOperator{\Wbhat}{\widehat{\Wb}}
\DeclareMathOperator{\Xbhat}{\widehat{\Xb}}
\DeclareMathOperator{\Ybhat}{\widehat{\Yb}}
\DeclareMathOperator{\Zbhat}{\widehat{\Zb}}

\DeclareMathOperator{\Acal}{\mathcal{A}}
\DeclareMathOperator{\Bcal}{\mathcal{B}}
\DeclareMathOperator{\Ccal}{\mathcal{C}}
\DeclareMathOperator{\Dcal}{\mathcal{D}}
\DeclareMathOperator{\Ecal}{\mathcal{E}}
\DeclareMathOperator{\Fcal}{\mathcal{F}}
\DeclareMathOperator{\Gcal}{\mathcal{G}}
\DeclareMathOperator{\Hcal}{\mathcal{H}}
\DeclareMathOperator{\Ical}{\mathcal{I}}
\DeclareMathOperator{\Jcal}{\mathcal{J}}
\DeclareMathOperator{\Kcal}{\mathcal{K}}
\DeclareMathOperator{\Lcal}{\mathcal{L}}
\DeclareMathOperator{\Mcal}{\mathcal{M}}
\DeclareMathOperator{\Ncal}{\mathcal{N}}
\DeclareMathOperator{\Ocal}{\mathcal{O}}
\DeclareMathOperator{\Pcal}{\mathcal{P}}
\DeclareMathOperator{\Qcal}{\mathcal{Q}}
\DeclareMathOperator{\Rcal}{\mathcal{R}}
\DeclareMathOperator{\Scal}{\mathcal{S}}
\DeclareMathOperator{\Tcal}{\mathcal{T}}
\DeclareMathOperator{\Ucal}{\mathcal{U}}
\DeclareMathOperator{\Vcal}{\mathcal{V}}
\DeclareMathOperator{\Wcal}{\mathcal{W}}
\DeclareMathOperator{\Xcal}{\mathcal{X}}
\DeclareMathOperator{\Ycal}{\mathcal{Y}}
\DeclareMathOperator{\Zcal}{\mathcal{Z}}

\DeclareMathOperator{\Atilde}{\widetilde{A}}
\DeclareMathOperator{\Btilde}{\widetilde{B}}
\DeclareMathOperator{\Ctilde}{\widetilde{C}}
\DeclareMathOperator{\Dtilde}{\widetilde{D}}
\DeclareMathOperator{\Etilde}{\widetilde{E}}
\DeclareMathOperator{\Ftilde}{\widetilde{F}}
\DeclareMathOperator{\Gtilde}{\widetilde{G}}
\DeclareMathOperator{\Htilde}{\widetilde{H}}
\DeclareMathOperator{\Itilde}{\widetilde{I}}
\DeclareMathOperator{\Jtilde}{\widetilde{J}}
\DeclareMathOperator{\Ktilde}{\widetilde{K}}
\DeclareMathOperator{\Ltilde}{\widetilde{L}}
\DeclareMathOperator{\Mtilde}{\widetilde{M}}
\DeclareMathOperator{\Ntilde}{\widetilde{N}}
\DeclareMathOperator{\Otilde}{\widetilde{O}}
\DeclareMathOperator{\Ptilde}{\widetilde{P}}
\DeclareMathOperator{\Qtilde}{\widetilde{Q}}
\DeclareMathOperator{\Rtilde}{\widetilde{R}}
\DeclareMathOperator{\Stilde}{\widetilde{S}}
\DeclareMathOperator{\Ttilde}{\widetilde{T}}
\DeclareMathOperator{\Utilde}{\widetilde{U}}
\DeclareMathOperator{\Vtilde}{\widetilde{V}}
\DeclareMathOperator{\Wtilde}{\widetilde{W}}
\DeclareMathOperator{\Xtilde}{\widetilde{X}}
\DeclareMathOperator{\Ytilde}{\widetilde{Y}}
\DeclareMathOperator{\Ztilde}{\widetilde{Z}}


%%%%%%%% Widely accepted definitions %%%%%%%%%%%%%%%

\DeclareMathOperator{\CC}{\mathbb{C}} % Complex numbers
\DeclareMathOperator{\EE}{\mathbb{E}} % Expectation
\DeclareMathOperator{\KK}{\mathbb{K}} % Arbitrary field
\DeclareMathOperator{\MM}{\mathbb{M}} % Median
\DeclareMathOperator{\NN}{\mathbb{N}} % Natural numbers
\DeclareMathOperator{\PP}{\mathbb{P}} % Probability
\DeclareMathOperator{\QQ}{\mathbb{Q}} % Rationals
\DeclareMathOperator{\RR}{\mathbb{R}} % Real numbers
\DeclareMathOperator{\ZZ}{\mathbb{Z}} % Integers
\DeclareMathOperator{\II}{\mathbb{I}}
\DeclareMathOperator{\VV}{\mathbb{V}}


\DeclareMathOperator{\one}{\mathbf{1}}  % Identity
\DeclareMathOperator{\zero}{\mathbf{0}} % Zero

\DeclareMathOperator*{\mini}{\mathop{\mathrm{minimize}}}
\DeclareMathOperator*{\maxi}{\mathop{\mathrm{maximize}}}
\DeclareMathOperator*{\argmin}{\mathop{\mathrm{argmin}}}
\DeclareMathOperator*{\argmax}{\mathop{\mathrm{argmax}}}
\DeclareMathOperator{\sgn}{\mathop{\mathrm{sign}}}
\DeclareMathOperator{\tr}{\mathop{\mathrm{tr}}}
\DeclareMathOperator{\rank}{\mathop{\mathrm{rank}}}
\DeclareMathOperator{\traj}{\mathop{\mathrm{Traj}}}
\DeclareMathOperator{\diag}{diag}


%%%%%%%% Bold Greek Letters %%%%%%%%%%%%%%%
% \DeclareMathOperator{\alphab}{{\bm{\alpha}}}
% \DeclareMathOperator{\betab}{{\bm{\beta}}}
% \DeclareMathOperator{\gammab}{{\bm{\gamma}}}
% \DeclareMathOperator{\deltab}{{\bm{\delta}}}
% \DeclareMathOperator{\epsilonb}{{\bm{\epsilon}}}
% \DeclareMathOperator{\varepsilonb}{{\bm{\varepsilon}}}
% \DeclareMathOperator{\zetab}{{\bm{\zeta}}}
% \DeclareMathOperator{\etab}{{\bm{\eta}}}
% \DeclareMathOperator{\thetab}{{\bm{\theta}}}
% \DeclareMathOperator{\varthetab}{{\bm{\vartheta}}}
% \DeclareMathOperator{\kappab}{{\bm{\kappa}}}
% \DeclareMathOperator{\lambdab}{{\bm{\lambda}}}
% \DeclareMathOperator{\mub}{{\bm{\mu}}}
% \DeclareMathOperator{\nub}{{\bm{\nu}}}
% \DeclareMathOperator{\xib}{{\bm{\xi}}}
% \DeclareMathOperator{\pib}{{\bm{\pi}}}
% \DeclareMathOperator{\varpib}{{\bm{\varpi}}}
% \DeclareMathOperator{\rhob}{{\bm{\rho}}}
% \DeclareMathOperator{\varrhob}{{\bm{\varrho}}}
% \DeclareMathOperator{\sigmab}{{\bm{\sigma}}}
% \DeclareMathOperator{\varsigmab}{{\bm{\varsigma}}}
% \DeclareMathOperator{\taub}{{\bm{\tau}}}
% \DeclareMathOperator{\upsilonb}{{\bm{\upsilon}}}
% \DeclareMathOperator{\phib}{{\bm{\phi}}}
% \DeclareMathOperator{\varphib}{{\bm{\varphi}}}
% \DeclareMathOperator{\chib}{{\bm{\chi}}}
% \DeclareMathOperator{\psib}{{\bm{\psi}}}
% \DeclareMathOperator{\omegab}{{\bm{\omega}}}

\DeclareMathOperator{\alphab}{{\mathbold{\alpha}}}
\DeclareMathOperator{\betab}{{\mathbold{\beta}}}
\DeclareMathOperator{\gammab}{{\mathbold{\gamma}}}
\DeclareMathOperator{\deltab}{{\mathbold{\delta}}}
\DeclareMathOperator{\epsilonb}{{\mathbold{\epsilon}}}
\DeclareMathOperator{\varepsilonb}{{\mathbold{\varepsilon}}}
\DeclareMathOperator{\zetab}{{\mathbold{\zeta}}}
\DeclareMathOperator{\etab}{{\mathbold{\eta}}}
\DeclareMathOperator{\thetab}{{\mathbold{\theta}}}
\DeclareMathOperator{\varthetab}{{\mathbold{\vartheta}}}
\DeclareMathOperator{\kappab}{{\mathbold{\kappa}}}
\DeclareMathOperator{\lambdab}{{\mathbold{\lambda}}}
\DeclareMathOperator{\mub}{{\mathbold{\mu}}}
\DeclareMathOperator{\nub}{{\mathbold{\nu}}}
\DeclareMathOperator{\xib}{{\mathbold{\xi}}}
\DeclareMathOperator{\pib}{{\mathbold{\pi}}}
\DeclareMathOperator{\varpib}{{\mathbold{\varpi}}}
\DeclareMathOperator{\rhob}{{\mathbold{\rho}}}
\DeclareMathOperator{\varrhob}{{\mathbold{\varrho}}}
\DeclareMathOperator{\sigmab}{{\mathbold{\sigma}}}
\DeclareMathOperator{\varsigmab}{{\mathbold{\varsigma}}}
\DeclareMathOperator{\taub}{{\mathbold{\tau}}}
\DeclareMathOperator{\upsilonb}{{\mathbold{\upsilon}}}
\DeclareMathOperator{\phib}{{\mathbold{\phi}}}
\DeclareMathOperator{\varphib}{{\mathbold{\varphi}}}
\DeclareMathOperator{\chib}{{\mathbold{\chi}}}
\DeclareMathOperator{\psib}{{\mathbold{\psi}}}
\DeclareMathOperator{\omegab}{{\mathbold{\omega}}}


\DeclareMathOperator{\sigmah}{{\widehat{\sigma}}}
\DeclareMathOperator{\lambdah}{{\widehat{\zeta}}}
\DeclareMathOperator{\psih}{{\widehat{\psi}}}


% \DeclareMathOperator{\Gammab}{{\bm{\Gamma}}}
% \DeclareMathOperator{\Deltab}{{\bm{\Delta}}}
% \DeclareMathOperator{\Thetab}{{\bm{\Theta}}}
% \DeclareMathOperator{\Lambdab}{{\bm{\Lambda}}}
% \DeclareMathOperator{\Xib}{{\bm{\Xi}}}
% \DeclareMathOperator{\Pib}{{\bm{\Pi}}}
% \DeclareMathOperator{\Sigmab}{{\bm{\Sigma}}}
% \DeclareMathOperator{\Upsilonb}{{\bm{\Upsilon}}}
% \DeclareMathOperator{\Phib}{{\bm{\Phi}}}
% \DeclareMathOperator{\Psib}{{\bm{\Psi}}}
% \DeclareMathOperator{\Omegab}{{\bm{\Omega}}}

\DeclareMathOperator{\Gammab}{{\mathbold{\Gamma}}}
\DeclareMathOperator{\Deltab}{{\mathbold{\Delta}}}
\DeclareMathOperator{\Thetab}{{\mathbold{\Theta}}}
\DeclareMathOperator{\Lambdab}{{\mathbold{\Lambda}}}
\DeclareMathOperator{\Xib}{{\mathbold{\Xi}}}
\DeclareMathOperator{\Pib}{{\mathbold{\Pi}}}
\DeclareMathOperator{\Sigmab}{{\mathbold{\Sigma}}}
\DeclareMathOperator{\Upsilonb}{{\mathbold{\Upsilon}}}
\DeclareMathOperator{\Phib}{{\mathbold{\Phi}}}
\DeclareMathOperator{\Psib}{{\mathbold{\Psi}}}
\DeclareMathOperator{\Omegab}{{\mathbold{\Omega}}}

\DeclareMathOperator{\Gammacal}{{\mathcal{\Gamma}}}
\DeclareMathOperator{\Deltacal}{{\mathcal{\Delta}}}
\DeclareMathOperator{\Thetacal}{{\mathcal{\Theta}}}
\DeclareMathOperator{\Lambdacal}{{\mathcal{\Lambda}}}
\DeclareMathOperator{\Xical}{{\mathcal{\Xi}}}
\DeclareMathOperator{\Pical}{{\mathcal{\Pi}}}
\DeclareMathOperator{\Sigmacal}{{\mathcal{\Sigma}}}
\DeclareMathOperator{\Upsiloncal}{{\mathcal{\Upsilon}}}
\DeclareMathOperator{\Phical}{{\mathcal{\Phi}}}
\DeclareMathOperator{\Psical}{{\mathcal{\Psi}}}
\DeclareMathOperator{\Omegacal}{{\mathcal{\Omega}}}

%%%%%%%% Mess around with LaTeX %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\newtheorem{theorem}{Theorem}[section]
\newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{hypothesis}[theorem]{Hypothesis}
\newtheorem{assumption}[theorem]{Assumption}

\newtheorem{lemma}{Lemma}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{question}[theorem]{Question}

%\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
%\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
\fi

% % \ifx\theorem\undefined
% % \newtheorem{theorem}{Theorem}
% % \fi
% \ifx\example\undefined
% \newtheorem{example}{Example}
% \fi
% % \ifx\lemma\undefined
% % \newtheorem{lemma}[theorem]{Lemma}
% % \fi

% \ifx\corollary\undefined
% \newtheorem{corollary}[theorem]{Corollary}
% \fi

% \ifx\definition\undefined
% \newtheorem{definition}[theorem]{Definition}
% \fi

% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{remark}[theorem]{Remark}
% \newtheorem{conjecture}[theorem]{Conjecture}

% \newtheorem{factoid}[theorem]{Fact}

% \ifx\axiom\undefined
% \newtheorem{axiom}[theorem]{Axiom}
% \fi

%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\sembrack}[1]{[\![#1]\!]}

%brackets
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}

\newcommand{\ea}{\emph{et al. }}
\newcommand{\eg}{\emph{e.g. }}
\newcommand{\ie}{\emph{i.e., }}

\newcommand{\sri}[1]{\textcolor{red}{{\slshape #1}}}

%Logic
% \newcommand{\implies}{\Rightarrow}
% \newcommand{\iff}{\Leftrightarrow}
\newcommand{\goesto}{\rightarrow}
\newcommand{\suchthat}{\ensuremathmode{\text{ such that }}}
%\newcommand{\st}{\suchthat}

%%%%%%%% Specific symbols for this project %%%%%%%%%%%%%%%

% upright names for matrices --don't use for single-letter function names!
\DeclareMathOperator{\DD}{\mathbb{D}} % DD
\DeclareMathOperator{\Thetabb}{\mathcal{C}} % DD

% Dual Spaces
\DeclareMathOperator{\Xcals}{\Xcal^{*}}
\DeclareMathOperator{\Mcals}{\Mcal^{*}}

% set and domain concepts
\DeclareMathOperator{\ri}{\mathrm{ri}}      % Relative interior
\DeclareMathOperator{\intr}{\mathrm{int}}   % Interior
\DeclareMathOperator{\bd}{\mathrm{bdry}}      % Boundary (see RocWet98)
\DeclareMathOperator{\dom}{\mathrm{dom}}    % Effective Domain
\DeclareMathOperator{\epi}{\mathrm{epi}}    % Epigraph
\DeclareMathOperator{\ran}{\mathrm{range}}  % Range of an operator

\newcommand{\by}{\times}

% gradient: \grad{F}{\m}
\newcommand{\grad}[2]{\nabla #1 \left( #2 \right) }
\newcommand{\hess}[2]{\nabla^2 #1 \left( #2 \right) }
\newcommand{\grd}{\nabla} % simpler version!
\newcommand{\breg}[1]{\Delta #1} % Bregman divergence

% subgradient: \subgrad{F}{\m}
\newcommand{\subgrad}[2]{\partial #1 \left( #2 \right) }
% subdiferential
\newcommand{\subdiff}{\partial}

% Vector of all ones
\newcommand{\ones}{\eb}

% Sum from i equal 1 to n
\newcommand{\sumin}{\sum_{i=1}^{n}}
\newcommand{\sumjn}{\sum_{j=1}^{n}}

% Deformed logarithm wrt \phi
\newcommand{\lphi}{\log_{\phi}}

% function k_{\phi}
\newcommand{\kphi}{k_{\phi}}

% reparam for dual log
\newcommand{\phibl}{\phi^{\bullet}}
\newcommand{\psibl}{\psi^{\bullet}}

% Deformed exponential wrt \phi
\newcommand{\ephi}{\exp_{\phi}}

% One over deformed exponential wrt \phi
\newcommand{\ephibl}{\exp^{\bullet}_{\phi}}

% Gradient of deformed exponential wrt \phi
\newcommand{\ephip}{\nabla_{x} \exp_{\phi}}

% Gradient of t-exponential wrt \phi
\newcommand{\ephit}{\nabla_{x} \exp_{t}}

% Deformed logarithm wrt \psi
\newcommand{\lpsi}{\log_{\psi}}

% One over deformed logarithm wrt \psi
\newcommand{\lpsib}{\log^{\bullet}_{\psi}}
\newcommand{\lphibl}{\log^{\bullet}_{\phi}}

%composition needed for conjugate--formerly combo
\newcommand{\lcirce}{\lpsi \circ \ephibl}

% S and related
\newcommand{\Sp}{S_{\phi}}
\newcommand{\Sps}{S^{*}_{\phi}}
\newcommand{\smp}{s_{\phi}}
\newcommand{\smpp}{s^{\prime}_{\phi}}
\newcommand{\smps}{s^{*}_{\phi}}

% T
\DeclareMathOperator{\tp}{\tilde{p}}
\DeclareMathOperator{\tq}{\tilde{q}}
\DeclareMathOperator{\tg}{\tilde{g}}
\DeclareMathOperator{\tmu}{\tilde{\mu}}
\DeclareMathOperator{\tthe}{\tilde{\theta}}
\DeclareMathOperator{\ttheb}{\tilde{\mathbf{\theta}}}
\DeclareMathOperator{\tmc}{\widehat{\Mcal}}
\DeclareMathOperator{\tv}{\tilde{v}}

\DeclareMathOperator{\Remp}{R_{\text{emp}}}

